The Unreasonable Effectiveness of Greedy Algorithms in Multi-Armed Bandit with Many Arms

We investigate a Bayesian $k$-armed bandit problem in the \emph{many-armed} regime, where $k \geq \sqrt{T}$ and $T$ represents the time horizon. Initially, and aligned with recent literature on many-armed bandit problems, we observe that subsampling plays a key role in designing optimal algorithms; the conventional UCB algorithm is sub-optimal, whereas a subsampled UCB (SS-UCB), which selects $\Theta(\sqrt{T})$ arms for execution under the UCB framework, achieves rate-optimality. However, despite SS-UCB's theoretical promise of optimal regret, it empirically underperforms compared to a greedy algorithm that consistently chooses the empirically best arm. This observation extends to contextual settings through simulations with real-world data. Our findings suggest a new form of \emph{free exploration} beneficial to greedy algorithms in the many-armed context, fundamentally linked to a tail event concerning the prior distribution of arm rewards. This finding diverges from the notion of free exploration, which relates to covariate variation, as recently discussed in contextual bandit literature. Expanding upon these insights, we establish that the subsampled greedy approach not only achieves rate-optimality for Bernoulli bandits within the many-armed regime but also attains sublinear regret across broader distributions. Collectively, our research indicates that in the many-armed regime, practitioners might find greater value in adopting greedy algorithms.

==> acknowledgements.tex <==
\section*{Acknowledgements}\label{sec:acknowledgements}
This work was supported by the Stanford Human-Centered AI Institute, and by the National Science Foundation under grants 1931696,  1839229, and 1554140.

==> conclusion.tex <==
%\section{Conclusion}
%\label{sec:conclusion}

%\vspace{5mm}
%\paragraph{Conclusion.}

%% Besides characterizing fundamental lower bounds and providing optimal algorithms, we also noted that the greedy algorithm empirically performed surprisingly well in this setting.  We provided theoretical analysis to explain this performance.

%% Our work naturally inspires several followup directions; we highlight two.  First, our analysis is carried out in a non-contextual setting; it is natural to extend our analysis to the contextual setting with many arms, where greedy algorithms have previously been seen to perform well even with a fixed number of arms.  Second, we believe our work motivates investigation of a number of refinements to greedy algorithms; e.g., those that subsample, or those that adaptively determine when to try a new arm.  We leave these directions for future work.




==> greedy_mod.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Analysis of A Greedy Algorithm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{A Greedy Algorithm}\label{sec:greedy}

Motivated by the performance observed in Figure \ref{fig:alph_60} as described in the introduction (and further elaborated in our simulations below), in this section we characterize performance of a {\em greedy} algorithm.  The greedy algorithm pulls each arm once and from then starts pulling the arm with the highest estimated mean; the formal definition follows.
%% We denote the estimated mean of arm $i$ at time $t$ by $\widehat{\mu}_{i}(t)$ which is defined as
%% \begin{equation*}
%%     \widehat{\mu}_{i}(t) = \frac{\sum_{s=1}^{t} Y_{is} \Ind \bp{\pi_s = i}}{N_i(t)},
%% \end{equation*}
%% where $a_s$ denotes the arm pulled at time $s$. Recall that $N_i(t-1) = \sum_{s=1}^{t-1} \Ind_{\bc{a_s = i}}$ is the number of times that arm $i$ has been pulled before time $t$. Therefore, at any time after $t \geq k+1$, the greedy algorithm pulls the arm which maximizes $\widehat{\mu}_{i}(t-1)$.

\begin{algorithm}
\caption{Greedy Algorithm}\label{alg:greedy}
\begin{algorithmic}[1]
\STATE \textbf{Input:} $k$
\FOR {$t \leq k$}
\STATE Pull arm $a_t = t$
\ENDFOR
\FOR {$t \geq k+1$}
\STATE Pull arm $a_t = \argmax_{i} \hmu_i(t-1)$
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Upper Bound on Bayesian Regret}

We derive an upper bound on the performance of the greedy algorithm described in Algorithm \ref{alg:greedy}. The main technical arguments in the proof involve bounding the probability that for a near-optimal arm $i$, the estimated mean of  $\hmu_i(t-1)$ falls below $\mu_i - \delta$, for $\delta > 0$.  To start, we first state a result that shows how such a bound can be used to provide an upper bound on Bayesian regret.

\begin{lemma}[\textbf{Generic bounds on Bayesian regret of greedy}]\label{lem:greedy-gen}
Let assumptions \ref{ass:prior} and \ref{ass:reward} hold. Furthermore, suppose that there exist a function $h(\cdot)$ and a constant $\vep_0$ such that for any $\vep \leq \vep_0$ the following holds: for any $\mu \geq 1-\vep$ and $\delta >0$, for a sequence of i.i.d.~samples $\bc{X_i}_{i=1}^n$ with $X_i \sim P_\mu$, we have
%
\begin{equation}\label{eqn:max-cross}
\P \bb{\exists~n: M_n < \mu - \delta } \leq \exp \bp{-h(\delta)}\,,
\end{equation}
%
where $M_n = \sum_{i=1}^n X_i/n$. Let $C_1 = (1-\exp(-1))/2$. Then, for any $\vep \leq \vep_0$, the following bound on Bayesian regret of greedy holds:
%
\begin{align}\label{eqn:reg-greedy}
BR_T & (\text{greedy}) \leq  T \bb{\frac{4}{\vep} \exp \bp{-\frac{k c_0 \vep}{12}} + \exp \bp{\frac{-k c_0 h(\vep) \vep}{2} }}  \nonumber \\
&+ 3T\vep + k \bp{1+\frac{9C_0}{2C_1}} + \frac{9k C_0}{2 C_1} \log \bp{\frac{1}{\vep}} \,.
\end{align}
\end{lemma}
%
%\begin{lemma}\label{lem:max-crossing}
%    Let $\bc{Z_i}_{i=1}^\infty$ be a sequence of i.i.d. random variables distributed according to $Q$. Suppose that $\E[Z_i] = \delta > 0$ and that $Z_i - \delta$ is $1$-subgaussian. Define $a_n = \sup_{n=1}^{\infty} P[Z_i \geq 1/n]^n$ and $b_n = \E[Z_i \Ind(Z_i \geq 0)]$. Then, for any $\delta \leq 0.05$ we have
%    \begin{align*}
%        \IP{\exists~n: M_n<\theta}
%        \leq
%        \exp\bp{-\frac{a_\mu}{e} \delta}\,.
%    \end{align*}
    %provided that $\delta \leq \frac{2\sqrt{2}}{\pi}$. Here $\Phi(z) = \int_{-\infty}^z \frac{1}{\sqrt{2 \pi}}\exp(-x^2/2) dx$ is the CDF of the standard normal variable.
%\end{lemma}
%
The preceding lemma is the key technical result in the analysis of greedy algorithm. As can be observed, the value of $\vep$ should be chosen to satisfy $h(\vep) \vep \geq 2 \log T/ (c_0 k)$ in order to make sure the third term in the regret term is sub-linear in $T$. If such a choice of $\vep$ is used, it is easy to see that the first two terms in the regret are bounded above by a constant and therefore the dominant terms are the third and the last term. For such a choice, the upper bound reduces to:
\begin{equation*}
3T \vep + \frac{9k C_0}{2 C_1} \log(1/\vep) ~\text{~~~for~~~} \vep h(\vep) \geq \frac{2 \log T}{c_0 k} \,,
\end{equation*}
for some constants $C_0$ and $C_1$.  Therefore, the best bound is obtained by choosing $\vep = \vep^*$ which is the smallest value of $\vep$ that satisfies the above condition, i.e., $\vep^* = \inf \bc{\vep: \vep h(\vep) \geq 2 \log T/(c_0 k)}$.

This is the approach we leverage in our analysis of the greedy algorithm; in particular, the shape of $h$ will dictate the quality of the upper bound obtained.  In turn, $h$ depends on the family of reward distributions being considered.  In the remainder of the section, we provide two upper bounds on Bayesian regret of the greedy algorithm.  The first only requires the assumption that the reward distribution is $1$-subgaussian; this leads to an $h(\delta)$ that is quadratic.  The second upper bound makes an additional (mild) assumption on the reward distribution; this leads to an $h(\delta)$ that is linear, and as a result, a better upper bound on regret.

Next, we need to find the relevant function $h(\delta)$ that appears in \eqref{eqn:max-cross}.  In the general case of a $1$-subgaussian reward distribution, we have the following lemma.

\begin{lemma}\label{lem:subg-crossing}
Let $Q$ be a distribution with mean $\mu$ such that $Q - \mu$ is $1$-subgaussian. Let $\bc{X_i}_{i=1}^n$ be i.i.d samples from distribution $Q$, $S_n = \sum_{i=1}^n X_i$ and $M_n= S_n / n$. Then for any $\delta > 0$, we have
\begin{equation}\label{eqn:subg-bound}
\P \bb{\exists~n: M_n < \mu - \delta } \leq \exp \bp{-\delta^2/2} \,.
\end{equation}
\end{lemma}

In other words, for a general $1$-subgaussian reward distribution, we have $h(\delta) = \delta^2/2$.  We develop a proof for the preceding lemma using {\em Lundberg's inequality} from ruin analysis of random walks, which is stated below.  This proof technique proves to be useful in our subsequent development.  The proof of Lemma \ref{lem:subg-crossing} is provided in Appendix \ref{app:greedy-proofs}.

\begin{proposition}[Lundberg's Inequality]\label{prop:lundberg}
Let $X_1, X_2, \ldots$ be a sequence of i.i.d.~samples from distribution $Q$. Let $S_n = \sum_{i=1}^n X_i$ and $S_0 = 0$. For any $u>0$ define the stopping time $\eta(u) = \inf \bc{n \geq 0: S_n > u}$
% (note that in risk theory, usually the random walk $u-S_n$ is considered and $\eta(u)$ is probability of hitting $0$, i.e., ruin)
 and let $\psi(u)$ denote the probability $\psi(u) = \P[\eta(u) < \infty]$. Assume there is a $\gamma > 0$ such that $\E[\exp(\gamma X_1)] = 1$
% (this is called the adjustment coefficient for distribution $Q$)
and that $S_n \stackrel{\text{a.s.}}{\longrightarrow} -\infty$ on the set $\bc{\eta(u) = \infty}$. Then,
$\psi(u) \leq \exp(-\gamma u)$.
\end{proposition}
The proof of Lundberg's inequality follows from applying the optional stopping theorem to martingale $\exp(\gamma S_n)$ for stopping time $\eta(u)$. For more details, see Corollary 3.4 of \cite{asmussen2010ruin}. 

Combining Lemmas \ref{lem:greedy-gen} \& \ref{lem:subg-crossing}, we obtain the following result.
%
\begin{theorem}\label{thm:greedy-reg-1sg}
Let assumptions \ref{ass:prior} and \ref{ass:reward} hold. Suppose that the greedy algorithm (Algorithm \ref{alg:greedy}) is executed. Let $C_1 = (1-\exp(-1))/2$. Then, for any $k \geq 4 \log T/c_0$, the Bayesian regret of the greedy algorithm satisfies 
\begin{align*}
&BR_T(\text{greedy}) \leq 4T \bp{\frac{k c_0}{4 \log T}}^{\frac{1}{3}} \exp \bp{-\frac{1}{12} \bb{\frac{k^2 c_0^2}{4 \log T}}^{\frac{1}{3}}}  \\
&~+ 3T \bp{\frac{4 \log T}{k c_0}}^{\frac{1}{3}} + k (1+\frac{9C_0}{2C_1}) + \frac{3k C_0}{2 C_1} \log \bp{\frac{k c_0}{4 \log T}} \\
&~=O \bp{\max \bb{T \bp{\frac{\log T}{k}}^{\frac{1}{3}}, k \log \log k}} \,.
\end{align*}
\end{theorem}
%
\begin{proof}
Note that the result of Lemma \ref{lem:subg-crossing} holds for all $1$-subgaussian distributions. Therefore, we can apply Lemma \ref{lem:greedy-gen} for $h(\vep) = \vep^2/2$ and $\vep_0 = 1$. In particular, substituting $\vep = (\frac{4 \log T}{k c_0})^{1/3}$ in this Equation \eqref{eqn:reg-greedy} proves the first result. The condition on $k$ implies that $\vep \leq \vep_0$. 
\end{proof}

%% Hence, Bayesian regret when the family of reward distributions satisfies Equation \ref{eqn:max-cross} for $h(\vep)$ which is linear function in terms of $\vep$ would scale as $\tilde{O} \bp{\max\bp{T/\sqrt{k}, k}}$. On the other hand, if the distribution only satisfies Equation \ref{eqn:max-cross} for $h(\vep)$ which is quadratic in terms of $\vep$, our upper bound on Bayesian regret of greedy would scale as $\tilde{O} \bp{\max \bp{T/\sqrt[3]{k},k}}$. This observation is formalized in the following theorem.

While the preceding upper bound on regret is appealing -- in particular, it is sublinear for any $\alpha \in (0,1]$ such that $k = T^\alpha$ --- we are motivated by the empirically strong performance of the greedy algorithm (cf.~Figure \ref{fig:alph_60}) to see if a stronger upper bound on regret is possible.  To this end, we make progress by showing that the achieved rate is further improvable for a large family of sub-gaussian reward distributions, including Gaussian and Bernoulli reward families. The following definition allows us to describe the reward families for which this improvement is feasible. 
%
\begin{definition}\label{def:upward-looking}
Let $Q$ be a distribution that satisfies $\E[Q] = \mu$ and that $Q - \mu$ is $1$-subgaussian. Let $\bc{X_i}_{i=1}^\infty$ be a sequence of i.i.d.~random variables distributed according to $Q$ and denote $S_n = \sum_{i=1}^n X_i$. For any $\theta < \mu$ define $R_n(\theta) = \sum_{i=1}^n X_i - n \theta$ and  $\tau(\theta) = \inf \{n \geq 1: R_n(\theta) < 0 \text{~or~} R_n (\theta) \geq 1\}$. We call the distribution $Q$ \textbf{upward-looking with parameter $p_0$} if for any $\theta < \mu$ one of the following conditions hold:

$\bullet$ $\P[R_{\tau(\theta)}(\theta) \geq 1] \geq p_0$.

$\bullet$ $\E[(X_1-\theta) \Ind(X_1 \geq \theta)] \geq p_0$. 

More generally, consider a family of distributions $\mathcal{Q} = \bc{Q_\mu: \mu \in [0,1]}$ that satisfy $\E[Q_\mu] = \mu$ and $Q_\mu-\mu$ is $1$-subgaussian. We call $\mathcal{Q}$ \textbf{uniformly upward-looking with parameters $(p_0, \delta_0)$} if all the distributions $Q_\mu, \mu \in [1-\delta_0, 1],$ are upward-looking with parameters $p_0$. 
\end{definition}
%
In Appendix \ref{app:examples}, we show that two classes of reward distributions are uniformly upward-looking. First, the class of all reward distributions $\mathcal{F}$ that for all $\mu \geq 1-\delta_0$ satisfy $\E[(X_\mu-\mu) \Ind(X_\mu \geq \mu)] \geq c_0$ for some constant $c_0$, are $(p_0, c_0)$ upward looking. This class includes the Gaussian reward distributions. The second class includes all reward distributions such that for all $\theta < \mu$, an integer $m \geq 1$ exists such that $\P[X_\mu \geq \theta + 1/m]^m \geq p_0$. This class includes the Bernoulli reward distributions.
 
%% To this end, we first state the following lemma.


%% Although the derived bound in \label{eqn:subg-bound} enables us to prove that the greedy algorithm achieves sub-linear Bayesian regret, 
%% In essence, the above definition asserts that the reward distributions put enough mass above the mean values of close to optimal arms, decreasing the probability that all such arms receive small rewards. This allows the greedy algorithm not to drop those optimal arms due to poor first few observations with a higher probability, hence getting a better regret performance.
%
The preceding discussion reveals that many natural families of reward distributions are upward-looking.  We now show that we can sharpen the result of Lemma \ref{lem:subg-crossing} for such distributions, as stated in the following lemma.   The proof is in Appendix \ref{app:greedy-proofs}.
%
\begin{lemma}\label{lem:max-crossing}
Let $Q$ be a distribution with mean $\mu$ which is upward-looking with parameter $p_0$ (See Definition \ref{def:upward-looking}). Let $\bc{X_i}_{i=1}^n$ be i.i.d samples from distribution $Q$, $S_n = \sum_{i=1}^n X_i$ and $M_n= S_n / n$. Then for any $\delta \leq 0.05$, we have
$\P \bb{\exists~n: M_n < \mu - \delta } \leq \exp \bp{-p_0 \delta/4}$.
\end{lemma}
%
Note that from this lemma, $h(\delta) = p_0 \delta/4$.  In our regime of interest, from Lemma \ref{lem:greedy-gen}, $\delta$ is chosen to be {\em small} (and indeed goes to zero as $k, T \rightarrow \infty$).   As a result, this {\em linear} $h(\delta)$ yields a strictly sharper upper bound on regret than a {\em quadratic} $h(\delta)$.  
%the former bound is strictly sharper. In order elaborate this more clearly, let us establish our generic regret bound on the performance of greedy algorithm.
%Note that the main difference between this result and the result of Lemma \ref{lem:max-crossing} is the power of $\delta$ inside the exponent. In other words, the latter one provides is $\exp(-c \delta)$ (sub-exponential) rather than $\exp(-c \delta^2)$ (sub-gaussian). As it becomes clear shortly, in our regime of interest that 
%$\delta$ will be chosen very small 
%
%
\begin{theorem}\label{thm:greedy-reg}
Let assumptions \ref{ass:prior} and \ref{ass:reward} hold.   Suppose also the family of reward distributions $\mathcal{F}$ is $(p_0, \delta_0)$ uniformly upward-looking.  Suppose that the greedy algorithm (Algorithm \ref{alg:greedy}) is executed. Let $C_1 = (1-\exp(-1))/2$. Then for any $k \geq \frac{8 \max \bp{400, 1/\delta_0^2}}{c_0 p_0} \log T$, the Bayesian regret of the greedy algorithm satisfies:
\begin{align*}
BR_T(\text{greedy}) &\leq T \sqrt{\frac{2 k c_0 p_0}{\log T}} e^{-\sqrt{k \log T} \sqrt{\frac{c_0}{18 p_0}}} + 1  \\
&+ 3T \sqrt{\frac{\log T}{8k c_0 p_0}} + k \bp{1+\frac{9C_0}{2C_1}} \\
&+ \frac{9k C_0}{4 C_1} \log \bp{\log{\frac{8k c_0 p_0}{\log T}}} \\
&=O \bp{\max \bb{T \bp{\frac{\log T}{k}}^{1/2}, k \log \log k}}\,.
\end{align*}
\end{theorem}
%
\begin{proof}
Note that Lemma \ref{lem:max-crossing} implies that for upward-looking distributions we can use Lemma \ref{lem:greedy-gen} for $h(\vep) = p_0 \vep/4$ and $\vep_0 = \min \bp{\delta_0, 0.05}$. Note that if $\delta_0 > 0.05$ and $\mathcal{F}$ is uniformly upward-looking with parameters $(p_0, \delta_0)$, so is for parameters $(p_0, 0.05)$. Hence, using the result of Lemma \ref{lem:greedy-gen}, by substituting $\vep = \sqrt{(8 \log T)/(k c_0 p_0)}$ in Equation \eqref{eqn:reg-greedy} implies the result. The condition on $k$ also implies that $\vep \leq \vep_0$ as desired.
\end{proof}
%
%Before proving this theorem we will state a lemma that is useful in our proof.
%\begin{lemma}\label{lem:max-crossing}
%    Let $(Y_i)_{i=1}^\infty$ be a sequence of random variables distributed according to $P_\mu$ which has mean $\mu$ and is $1$-subgaussian. Let $0<\theta<\mu$ be given and let $M_n$, denote the sample mean of $(Y_i)_{i=1}^n$. Define $Z_\mu = Y_1 - \mu$ which is $1$-subgaussian and $X_\mu = Z_\mu + (\mu - \theta)$. Then, the following holds:
%    \begin{equation*}
%        a_\mu = \E \bb{X_\mu \,\Ind \bp{X_\mu \geq 0}}\,,
%    \end{equation*}
%    Then, for any $\delta \leq 0.05$ we have
%    \begin{align*}
%        \IP{\exists~n: M_n<\theta}
%        \leq
%        \exp\bp{-\frac{a_\mu}{e} \delta}\,.
%    \end{align*}
    %provided that $\delta \leq \frac{2\sqrt{2}}{\pi}$. Here $\Phi(z) = \int_{-\infty}^z \frac{1}{\sqrt{2 \pi}}\exp(-x^2/2) dx$ is the CDF of the standard normal variable.
%\end{lemma}
%\begin{remark}
%Note that as proved in Lemma \ref{lem:max-crossing}, for all values of $\mu$, $a_\mu \geq \delta$ meaning that the bound $\exp(-\delta^2/e)$ holds for all $1$-subgaussian distributions. However, for many distributions $a_\mu$ has a constant lower bound. In fact, if there exist a positive constant $c_1$ such that for all $\mu \in [0,1]$ we have
%\begin{equation*}
%    \E[Z_\mu \Ind(Z_\mu \geq 0)] \geq c_1\,,
%\end{equation*}
%then it is easy to observe that $a_\mu \geq c_1$ and the bound becomes $\exp(-(c_1/e) \delta)$. As we observe later in Theorem \ref{thm:greedy-reg} the performance of greedy depends on whether this bound is sub-exponential vs sub-gaussian.
%\end{remark}\delta

\begin{comment}
\begin{proof}[Proof of Theorem \ref{thm:greedy-reg}]
Partition the interval $(0,1)$ into sub-intervals of size $\delta$. In particular, let $I_1, I_2, \ldots, I_h$ be defined as $I_i = (1-i\delta, 1-(i-1)\delta]$, where $h = \lceil{1/\delta \rceil}$. Let $N_i$ be the number of means $\mu$ that fall into the interval $I_i$. For any $1 \leq i \leq h$ and any $1 \leq j \leq k$, define $Z_{ij} = \Ind \bp{\mu_j \in I_i}$. Note that for any fixed $j$, $\bc{Z_{ij}}_{i=1}^k$ are independent Bernoulli variables satisfying $N_i = \sum_{j=1}^k Z_{ij}$ and $\IE{Z_{ij}} = p_i = \P \bp{\Gamma \in (1-i\delta, 1-(i-1)\delta]} \in [c_0 \delta, C_0 \delta]$ as the density of $\Gamma$ belongs to $[c_0,C_0]$. Therefore, using a Chernoff inequality for any $\theta \in (0,1)$ we have
\begin{equation*}
    \IP{\abs{\frac{N_i}{k}-p_i} \leq \theta p_i} \leq 2 \exp \bp{-k p_i \theta^2/3}
\end{equation*}
for any $\theta \leq 1/2$. Define $\mathcal{F} = \cap_{i=1}^h \bc{N_i \in [c_0 k \delta/2, 3C_0 k\delta/2]}$. Noting that $p_i \in [c_0, C_0]$, picking $\theta = 1/2$, and taking a union bound over $i \in [h]$ implies that
\begin{equation*}
\IP{\bar{\mathcal{F}}} \leq 2h \exp \bp{-k c_0 \delta/12} \leq \frac{4}{\delta} \exp \bp{-k c_0 \delta/12}\,.
\end{equation*}
Suppose that indices $n_1, n_2, \ldots, n_r \in [k]$ correspond to all arms that satisfy $\mu_{n_l} \geq 1-\delta$. For any $1 \leq l \leq r$, as $\mathcal[F]$ is upward-looking with parameters $(p_0,\vep)$ with $\delta \leq \vep$, Lemma \ref{lem:max-crossing} implies that
\begin{equation*}
\IP{\exists t: \hmu_{n_l}(t) < 1-2 \delta} \leq \exp\bp{-\frac{p_0 \delta}{4}}\,.
\end{equation*}
These events are independent for $1 \leq l \leq r$ and therefore if we define $\mathcal{\bar{G}} = \cap_{l: \mu_l \in I_1} \bc{\exists t: \hmu_l(t)<1-2 \delta}$ then
\begin{equation*}
\IP{\mathcal{\bar{G}} \cap \mathcal{F}} \leq \exp \bp{-N_1 \frac{p_0 \delta}{4}} \leq \exp \bp{-k \frac{c_0 p_0 \delta^2}{8}}\,.
\end{equation*}
Now the Bayesian regret can be written as
\begin{align}\label{eqn:bayes-regret}
BR_T(\bpi) &= \IE*{\bmu}{\sum_{\Delta_i>0} \Delta_i \IE{N_i(T) \mid \bmu}} \nonumber \\
&\leq T \bc{\IP{\mathcal{\bar{G}} \cap \mathcal{F}} + \IP{\mathcal{\bar{F}}}} \nonumber \\
&+ \IE*{\bmu}{\sum_{\Delta_i>0} \Delta_i \IE{N_i(T) \mid \bmu} \Ind{\bp{\mathcal{F} \cap \mathcal{G}}}}
\end{align}
where $N_i(t)$ denotes the total number of pulls for the sub-optimal arm $i$ and $\Delta_i = \mu^* - \mu_i$ is the gap for such an arm. Now suppose that both events $\mathcal{F}$ and $\mathcal{G}$ hold. We want to provide an upper bound on $\IE{N_i(T) \mid \bmu}$ for sub-optimal arms that have their means smaller than $1-3\delta$ (i.e., they belong to $I_4, I_5, \cdots, I_h$). Note that we pull each arm once and afterwards the arms are pulled using a greedy policy explained in Algorithm \ref{alg:greedy}. Since $\mathcal{G}$ and $\mathcal{F}$ hold, there exists at least one arm that has it's mean $\mu_j \in I_1$ and it's empirical estimate is always at least $1-2\delta$. Hence,
\begin{align*}
\IP{N_i(T) \geq t + 1 \mid \bmu}
&\leq
\IP{\hmu_i(t) \geq 1- 2\delta \mid \bmu} \\
&\leq
%\IP{\Normal{\mu_i}{1/t} \geq 1-2\delta \mid \bmu}\\
%&\leq
\exp \bp{-t(1-2\delta-\mu_i)^2/2},
\end{align*}
where we used the fact that arm $i$ only would be pulled for the $t+1$ time if it's estimate after $t$ samples is larger than $1-2\delta$ and that (centered version of) $\hmu_i(t)$ is $1/t$-subgaussian. Now note that for any discrete random variable taking positive values $\IE{Z} = \sum_{t=1}^{\infty} \IP{Z \geq t}$ and therefore
\begin{align*}
\IE{N_i(T) \mid \bmu} 
&= 1 + \sum_{t \geq 1} \IP{N_i(T) \geq t+1 \mid \bmu} \\
&\leq 1 + \sum_{t=1}^{\infty} \exp\bp{\frac{-t(1-2\delta-\mu_i)^2}{2}} \\
&= 1 + \frac{1}{1-\exp \bp{\frac{(1-2\delta-\mu_i)^2}{2}}}
\end{align*}
Now note that for any $z \in [0,1]$ we have $\exp(-z) \leq 1 - 2cz$ where $C_1=(1-\exp(-1))/2$. Hence, we have
\begin{equation*}
\IE{N_i(T) \mid \bmu} \leq 1 + \frac{1}{C_1(1-2\delta-\mu_i)^2}\,,
\end{equation*}
which implies that
\begin{align*}
\Delta_i \IE{N_i(T) \mid \bmu} 
&\leq (1-\mu_i) + \frac{1-\mu_i}{C_1(1-2\delta-\mu_i)^2} \\
&\leq 1 + \frac{3}{C_1(1-2\delta-\mu_i)}\,,
\end{align*}
where we used the inequality that $1-\mu_i \leq 3(1-2\delta-\mu_i)$ as $\mu_i \leq 1-3\delta$. Now note that all above is true for any arm with mean that belongs to $\cup_{l=4}^h I_l$. Also, under the event $\mathcal{F}$ number of arms $N_l$ in each $I_l$ is at most $3C_0 k \delta/2$. Hence,
\begin{align*}
\sum_{l=4}^h & \sum_{i: \mu_i \in I_l} \Delta_i \IE{N_i(T) \mid \bmu} \Ind \bp{\mathcal{F} \cap \mathcal{G}} \\
&\leq \sum_{l=4}^h \sum_{i: \mu_i \in I_l} 1 + \bp{1+\frac{3}{C_1(1-2\delta-\mu_i)}} \\
&\leq k + \frac{3k C_0 \delta}{2} \sum_{l=4}^h \frac{1}{C_1 (l-3)\delta} \\
&\leq k + \frac{3k C_0}{2C_1} \sum_{l=1}^h \frac{1}{l} \\
&\leq k + \frac{3k C_0}{2C_1} (1+\log h) \\
&\leq k \bp{1+\frac{3C_0}{2C_1}} + \frac{3k C_0}{2 C_1} \log(1/\delta)\,.
\end{align*}
Finally, the total regret of arms that belong to $I_1, I_2$ and $I_3$ is upper bounded by $3T \delta$. Hence,
\begin{align*}
~~~~~&\IE*{\bmu}{\sum_{\Delta_i>0} \Delta_i \IE{N_i(T) \mid \bmu} \Ind\bp{\mathcal{F} \cap \mathcal{G}}} \\
& \leq 3T \delta + k \bp{1+\frac{3C_0}{2C_1}} + \frac{3k C_0}{2 C_1} \log(1/\delta)\,.
\end{align*}
Hence, replacing this in Equation \eqref{eqn:bayes-regret} we get
\begin{align*}
BR_T &\leq  T \bp{\frac{4}{\delta} \exp \bp{-k c_0 \delta/12} + \exp \bp{-k \frac{c_0 p_0 \delta^2}{8}} }  \\
&+ 3T\delta + k \bp{1+\frac{3C_0}{2C_1}} + \frac{3k C_0}{2 C_1} \log(1/\delta)\,.
\end{align*}
Putting $\delta = \sqrt{(8 \log T)/(k c_0 p_0)}$ which by our assumption is smaller than or equal to $\vep$ implies that
\begin{align*}
BR_T &\leq  T \bp{\sqrt{\frac{2 k c_0 p_0}{\log T}} \exp \bp{-\sqrt{k \log T} \sqrt{\frac{c_0}{18 p_0}}} + \frac{1}{T}}  \\
&+ 3T \sqrt{\frac{\log T}{8k c_0 p_0}} + k \bp{1+\frac{3C_0}{2C_1}} \\
&+ \frac{3k C_0}{4 C_1} \log \bp{\log{\frac{8k c_0 p_0}{\log T}}}
\end{align*}
Now looking at the above upper bound on Bayesian regret, it is not hard to see that in the regime of interest the first term goes to zero and hence the dominant terms are the third and the last term. This completes the proof of this theorem.
\end{proof}
\end{comment}
%


We conclude with the following corollary, that restates the preceding upper bound in terms of $\alpha$.
\begin{corollary}
Under assumptions \ref{ass:prior} and \ref{ass:reward}, if $k=\Theta \bp{T^{\alpha}}$, for uniformly upward-looking distributions we have:
\[
BR_T(\text{greedy}) = \left.
  \begin{cases}
    O(T^{1-\frac{\alpha}{2}}) \sqrt{\log T}, & \text{for } \alpha < 2/3 \\
    O(T^{\alpha} \log \log T), & \text{for } \alpha \geq 2/3
  \end{cases}
  \right. \,.
\]
\end{corollary}

